Posterior Re-calibration for Imbalanced Datasets

Neural Networks can perform poorly when the training label distribution is heavily imbalanced, as well as when the testing data differs from the training distribution. In order to deal with shift in the testing label distribution, which imbalance causes, we motivate the problem from the perspective of an optimal Bayes classifier and derive a post-training prior rebalancing technique that can be solved through a KL-divergence based optimization. This method allows a flexible post-training hyper-parameter to be efficiently tuned on a validation set and effectively modify the classifier margin to deal with this imbalance. We further combine this method with existing likelihood shift methods, re-interpreting them from the same Bayesian perspective, and demonstrating that our method can deal with both problems in a unified way. The resulting algorithm can be conveniently used on probabilistic classification problems agnostic to underlying architectures. Our results on six different datasets and five different architectures show state of art accuracy, including on large-scale imbalanced datasets such as iNaturalist for classification and Synthia for semantic segmentation. Please see https://github.com/GT-RIPL/UNO-IC.git for implementation.

==> figure/lambda_synthia.tex <==

\begin{figure}
\centering
\includegraphics[width=8cm]{figure/lambda_synthia.png}
 \caption{\textbf{Hyperparameter $\lambda$ search on Synthia validation set for imbalance calibration}. $\lambda = 0.0$ corresponds to the baseline performance. $\lambda = 0.4$ is used as the parameter for subsequent experiments on Synthia.} 
\label{fig:lambda}%
\end{figure} 

==> figure/synthia_rain_single.tex <==

\begin{figure}
\centering
\includegraphics[width=\linewidth]{figure/synthia_rain_single.png}
 \caption{\textbf{Qualitative result for Synthia Rain}. The rain condition is not seen during training. Our algorithm UNO-IC can capture fine details in segmentation even under severe viusal degradation not encounted during training. Our method combined with UNO demonstrates is effective against extreme dataset imbalance and unseen degradations in semantic segmentation.} 
\label{fig:synthia_rain_single}%
\end{figure} 

==> figure/unified_diagram.tex <==
\begin{figure}
\centering
\includegraphics[width=\linewidth]{figure/unified_diagram.png}
 \caption{}%
\label{fig:unified_diagram}%
\end{figure} 

==> impact.tex <==
\section*{Broader Impact}

Our work discusses a fundamental problem in deep learning: data imbalance. Data imbalance can be safety-critical in many applications such as self-driving. Our approach allows an algorithm to give more attention to pedestrians and small obstacles. Additionally, our unified algorithm aims to provide stable performance under severe visual degradation which is also critical for safty considerations.   

==> table/cifar_prec_save.tex <==
\begin{table}
\caption{\textbf{Top1 Precision}}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{c|cc|cc|cc|cc|cc|cc}  
\toprule
\multicolumn{1}{c|}{Dataset}  &\multicolumn{4}{c|}{Imbalanced CIFAR-10} &\multicolumn{4}{c|}{Imbalanced CIFAR-100}\\
\midrule
\multicolumn{1}{c|}{Imbalance Type} &\multicolumn{2}{c|}{long-tailed}
&\multicolumn{2}{c|}{step}  &\multicolumn{2}{c|}{long-tailed} &\multicolumn{2}{c|}{step} 
&AVE
&AVE*\\
\midrule
Imbalance Ratio & 100 & 10 & 100 & 10 & 100 & 10 & 100 & 10 \\
\midrule
ERM &71.52 &87.43 &65.99 & 85.46 &37.84& 56.79& 38.72& 54.67&62.30\\
Focal\cite{cao2019learning} &70.70 &86.48 &65.11 &85.08& 37.98& 56.40&38.51& 54.38&61.83\\
LDAM\cite{lin2017focal} &73.28 &86.23 &65.58& 84.67&40.30& 56.48& 39.41& 50.80 &62.09\\
\midrule\midrule
% CB RS&\\
CB ERM\cite{cui2019class}&73.23 &87.63 &62.57 &85.56 &32.07 &55.85 &19.6 &52.72\\
CB Focal\cite{cui2019class}&70.59 &86.94 &37.74 &84.87 &28.04 &54.83 & 8.87 & 50.09\\
\midrule\midrule
ERM-DRW &76.22 &88.15 &70.95 &87.21 &41.36&58.47& 44.30& 59.34&65.75\\
Focal-DRW &74.27 &88.00 &72.63 &88.18 &39.53&56.65&38.37&58.07&66.10\\
LDAM-DRW\cite{lin2017focal}& 76.62& 87.88& 77.31& 87.32 &42.23& 57.48&45.70&56.51&66.38\\
\midrule\midrule
ERM-MLF& $79.86_{2.1}$& $88.63_{0.7}$ &$74.39_{1.1}$ &$88.66_{1.0}$& $40.92_{1.3}$& $58.09_{1.0}$& $46.52_{1.2}$& $59.36_{1.3}$ &67.05\\
Focal-MLF&$80.16_{1.3}$ & $88.01_{1.1}$ &$74.32_{0.8}$ &$\mathbf{89.01_{1.0}}$& $41.65_{1.1}$& $57.99_{1.0}$& $\mathbf{47.27_{1.2}}$& $59.30_{1.0}$& 67.21\\
ERM-DRW-MLF&$\mathbf{81.09_{1.5}}$ &$\mathbf{88.56_{1.2}}$ &$\mathbf{78.55_{1.2}}$ &$88.58_{1.0}$ & $\mathbf{43.11_{0.6}}$ &$\mathbf{58.56_{0.5}}$ &$45.60_{0.3}$&$\mathbf{59.93_{0.3}}$&\textbf{68.00}\\
Focal-DRW-MLF&$78.37_{1.0}$ &$88.20_{0.5}$ &$78.37_{1.0}$ & $88.52_{0.5}$&$40.57_{0.5}$&$56.65_{0.0}$&$43.11_{0.6}$& $58.07_{0.0}$&66.48\\
\bottomrule
\end{tabular}}
\label{tab:cifar}
\end{table}

==> table/synthia.tex <==
\begin{table*}
\resizebox{\linewidth}{!}{%
\begin{tabular}{rr|rrr|rrr|rrr}  
\toprule
&\multicolumn{3}{C}{Building(30.1$\%$)} && \multicolumn{3}{c}{Pedestrian(0.6$\%$)} & \multicolumn{3}{c}{Bike(0.4$\%$)}\\
& & mIOU\uparrow & mACC\uparrow & mECE\downarrow &  mIOU\uparrow & mACC\uparrow & mECE\downarrow & mIOU\uparrow & mACC\uparrow & mECE\downarrow\\
\midrule
\multirow{3}{*}{Baseline}
ERM  &98.21$\pm$0.09 &99.22$\pm$0.04 &0.24  &76.63$\pm$0.63 &84.10$\pm$0.61 &9.31  &13.33$\pm$1.92 &15.67$\pm$2.31  &58.85\\
Focal
\midrule\midrule
\midrule
\multirow{2}{*}{ML}
&ERM-MLF $\lambda = 0.6$ &98.09$\pm$0.60 &98.90$\pm$0.07 &0.55 &75.18$\pm$0.65 &89.55$\pm$0.51 &6.09 &23.78$\pm$1.17 &83.22$\pm$4.01&5.71\\
\bottomrule
\end{tabular}}
\caption{\textbf{mIOU, mACC and mECE of the BGM and ML fusion on \textit{selected} Synthia classes}. This table compares the fusion algorithms with baselines on three classes: Building(30.1$\%$), Pedestrian(0.6$\%$) and Bike(0.4$\%$). The percentage indicates pixcel frequency in Sythina training set. Both ML and BGM improve accuracy on the minority classes.}
\label{tab:synthia_compare}
\end{table*}



